An Evolutionary Approach to Adapt Tests Across Mobile Apps

Automatic generators of GUI tests often fail to generate semantically relevant test cases, and thus miss important test scenarios. To address this issue, test adaptation techniques can be used to automatically generate semantically meaningful GUI tests from test cases of applications with similar functionalities. In this paper, we present ADAPTDROID, a technique that approaches the test adaptation problem as a search-problem, and uses evolutionary testing to adapt GUI tests (including oracles) across similar Android apps. In our evaluation with 32 popular Android apps, ADAPTDROID successfully adapted semantically relevant test cases in 11 out of 20 cross-app adaptation scenarios.

==> algs/fitnessAlg.tex <==
\begin{center}
\begin{algorithm}
\DontPrintSemicolon
\setlength{\algomargin}{-10mm}
\linespread{0.85}\selectfont
\SetAlCapHSkip{0em}
\SetKwProg{Fn}{function}{}{}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\Input{widgetMatches, GUIActions}
\Output{mappings}
\BlankLine
\Fn{\textbf{\textsc{computeMappings}}\emph{(widgetMatches, GUIActions)}}{
mappings $\leftarrow$ empty dictionary\;
possibleMappings $\leftarrow$ \textsc{allPossibleMatchCombinations}\emph{(widgetMatches,
  GUIActions)}\; 
\For{each possibleMapping $\in$ possibleMappings}{ 
\If{\textsc{areWidgetsMappedOnlyOnce}\emph{(possibleMapping)}$\wedge$
  \textsc{areMappedWidgetsNear}\emph{(possibleMapping)}$\wedge$\label{code:prune}}
{
mappings.add(possibleMapping)
}
}
\Return{mappings}
}
\Input{originalTest, evaluatedTest, widgetMatches}
\Output{similarityValue ([0 - 1])}
\BlankLine
\Fn{\textbf{\textsc{evaluateTestSimilarity}}\emph{(originalTest, evaluatedTest, widgetMatches)}}{
mappings $\leftarrow$ \textsc{computeMappings}\emph{(evaluatedTest.GUIActions, widgetMatches)}\label{code:mapping}\;
highestSimilarity $\leftarrow \varnothing$\; 
\For{\textbf{each} mapping $\in$ mappings\label{code:loop}}{
similarity $\leftarrow 0$\; 
matchedEventIndexes $\leftarrow$ empty dictionary\;
LOOP: \For{\textbf{each} originalEvent $\in$ originalTest.GUIEvents\label{code:events}}{
  matchedWidget $\leftarrow$ mapping[originalGUIEvent.widget]\;
  \If{matchedWidget $= \varnothing$\label{code:mapped}}{
    continue LOOP\;
  }
  index $\leftarrow$ \textsc{getHighestPastEventMatchIndex}\emph{(matchedEventIndexes,
  originalGUIEvent.pastEvents)}\label{code:index}\; 
  \eIf{originalEvent is GUIAction}{
    \For{i $\leftarrow$ index+1 \textbf{to} evaluatedTest.length\label{code:actions}}{
      action $\leftarrow$ evaluatedTest.GUIActions[i]\;
      \If{action.widget $=$ matchedWidget}{\tcp{The original GUI action is matched}
        \eIf{action is WriteGUIAction}{
          \eIf{action.typedText = originalEvent.typedText\label{code:write}}{
            similarity $\leftarrow$ similarity + 1\;
          }{
            similarity $\leftarrow$ similarity + 0.8\;
          }
     }{
        similarity $\leftarrow$ similarity + 1\;
     }
     matchedEventIndexes[originalEvent] $\leftarrow$ i\;
     continue LOOP\;
  }
}
}{
      \For{i  $\leftarrow$ index+1 \textbf{to} evaluatedTest.length+1\label{code:assertions}}{
        state $\leftarrow$ evaluatedTest.visitedStates[i]\;
        \If{(matchedWidget $\in$ state $\wedge$ originalEvent $\neq$ NotExistAssertion) $\lor$
          (matchedWidget.window = state.window $\wedge$ originalEvent = NotExistAssertion)}{\tcp{The
            original GUI assertion is matched}  
          similarity $\leftarrow$ similarity + 1 \;
          matchedEventIndexes[originalEvent] $\leftarrow$ i\;
          continue LOOP\;
        } 
        }
      }
    }
    highestSimilarity $\leftarrow$ \textsc{max}\emph{(similarity,
      highestSimilarity)}\label{code:heuristics}\; 
  }
  highestSimilarity $\leftarrow$ highestSimilarity +
  \textsc{nearMatchHeuristics}\emph{(evaluatedTest, widgetMatches)}\; 
\Return{highestSimilarity / originalTest.length}
}
\caption{Test case similarity algorithm}
\label{alg:fitness}
\end{algorithm}
\end{center}

==> algs/initPopAlg.tex <==
\begin{center}
\begin{algorithm}[t]
\DontPrintSemicolon
\setlength{\algomargin}{-10mm}
\linespread{0.85}\selectfont
\SetAlCapHSkip{0em}
\SetKwProg{Fn}{function}{}{}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\Input{$A_R$ recipient app, \textit{NR} $\#$ random tests, $L$ max test length}
\Output{$\mathcal{P}_0$ initial population}
\BlankLine
\Fn{ \textbf{\textsc{generateRandomPopulation}}\emph{($A_R$,\textit{NR},$L$)}}{

\While{$| \mathcal{P}_0 | <  \textit{NR}$ }{
	$t_R \leftarrow \varnothing$\;
	$S_0 \leftarrow $ open/restart $A_R$\tcp*{initial state}
	\For{i from  1 to L}{
			$e_i$$\leftarrow$\textsc{selectRandomEventEnabledIn}($S_{i-1}$)\tcp*{step 1}
		    add $e_i$ to $t_R$\tcp*{step 2}
		    $S_{i} \leftarrow $ execute $e_i$\tcp*{step 3}
		}
	add $t_R$ to $\mathcal{P}_0$\;
}
\Return{$\mathcal{P}_0$}
}
\vspace{-4mm}
\caption{Generation of \textit{NR} random tests in $\mathcal{P}_0$}

\label{alg:init}
\end{algorithm}
\end{center}


==> algs/orderigAlg.tex <==
\begin{center}
\begin{algorithm}[t]
\DontPrintSemicolon
\setlength{\algomargin}{-10mm}
\linespread{0.85}\selectfont
\SetAlCapHSkip{0em}
\SetKwProg{Fn}{function}{}{}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\Input{$t_D = \langle e_1,..., e_n\rangle$}
\Output{$\mathbb{C}$ set of clusters of events}
\BlankLine
\Fn{ \textbf{\textsc{computeClusterEvents}}\emph{($t_D$)}}{
$\mathbb{C} \leftarrow  \{ \}$ \tcp*{initiliaze the set of clusters}
c $\leftarrow  \{ e_1\} $ \tcp*{initiliaze the current cluster}
\For{i from  1 to n-1}{
\eIf{
\textsc{eventIsEnabledInState}\emph{($e_{i+1}$,$S_{i-i}$) $\land$ 
 \textsc{eventIsEnabledInState}\emph{($e_{i}$,$S_{i}$)} 
}} 
{
 add $\{ e_{i+1}\}$ to $c$ \tcp*{add $e_{i+1}$ to the current cluster}
}{
add c to $\mathbb{C}$ \tcp*{save the current cluster}
c $\leftarrow  \{e_{i+1}\}$ \tcp*{inizialize a new cluster with $e_{i+1}$}
}
}
add c to $\mathbb{C}$ \tcp*{save the current cluster}
\Return{$\mathbb{C}$}
}
\vspace{-4mm}
\caption{Events clustered based on ordering}

\label{alg:past}
\end{algorithm}
\end{center}


==> listings/AUTH.tex <==
{
\begin{lstlisting}[language=Alloy,caption={AUTH Abstract Semantics model}]
--------------------Initial State---------------
pred init [t: Time] {
	no Track.op.t
 	Currentwindow.isin.t = aws.Login
	\#List.elements.t = 0
}
---------------Generic AUTH Structure ----------
abstract sig Go, Login, Signup, Ok, Cancel, Logout extends Actionwidget { }
abstract sig User, Password, Usersave, Passwordsave, Repassword, Field extends Inputwidget { }

fact {
\#Tobecleaned=1
	not(User in Propertyrequired.requireds)
	not(Password in Propertyrequired.requireds)	
	not(Usersave in Propertyrequired.requireds)
	not(Passwordsave in Propertyrequired.requireds)
	not(Repassword in Propertyrequired.requireds)
}
---------------Generic AUTH Semantics---------- 
one sig Propertyrequired{
	requireds: set Inputwidget
}
sig Objectinlist extends Object{
	vs: Value lone -> Inputwidget
}
one sig List {
	elements: Objectinlist set -> Time
}
pred fillsemantics [iw: Inputwidget, t: Time, v: Value] { }
pred fillsuccesspost [iw: Inputwidget, t, t': Time, v: Value] {  
		List.elements.t' =  List.elements.t
}
pred fillfailpost [iw: Inputwidget, t, t': Time, v: Value] {
		List.elements.t' =  List.elements.t
}
pred fillpre[iw: Inputwidget, t: Time, v: Value] { 
	\#iw.content.(T/first) = 1 => not(v = none)
}
pred selectsemantics [sw: Selectablewidget, t: Time, o: Object] { }
pred selectsuccesspost [sw: Selectablewidget, t, t': Time, o: Object] { }
pred selectfailpost [sw: Selectablewidget, t, t': Time, o: Object] { }
pred selectpre[sw: Selectablewidget, t: Time, o: Object] { }

pred clicksemantics [aw: Actionwidget, t: Time] {
	(aw in Login) => filledlogintest [t] and existingtest [t] 
	(aw in Ok) => filledrequiredtest[t] and uniquefieldstest [t] and samepasstest [t]
}
pred clicksuccesspost [aw: Actionwidget, t, t': Time] {
	Currentwindow.isin.t' = aw.goes
	(aw in Ok) => add [t, t'] else List.elements.t' =  List.elements.t
	(all iw: Inputwidget | iw.content.t' = iw.content.(T/first))
}
pred clickfailpost [aw: Actionwidget, t, t': Time]	{
	(all iw: Inputwidget | iw.content.t' = iw.content.(T/first))
	List.elements.t' =  List.elements.t
}
pred clickpre[aw: Actionwidget, t: Time] { }
pred add [t, t': Time] {
	one o: Objectinlist |all iw: (Usersave + Passwordsave + Field) | not(o in List.elements.t) and o.appeared = t' and o.vs.iw = iw.content.t and List.elements.t' =  List.elements.t+o
}
pred filledlogintest [t: Time] {
	all iw: (User+Password)| \#iw.content.t = 1   and not(iw.content.t=Tobecleaned)
}
pred existingtest [t: Time] {
	one o: List.elements.t | Password.content.t =o.vs.Passwordsave and User.content.t =o.vs.Usersave
}
pred samepasstest [t: Time] {
	Passwordsave.content.t = Repassword.content.t
}
pred filledrequiredtest [t: Time] {
 	\#Usersave.content.t = 1 and not(Usersave.content.t=Tobecleaned) 
 	\#Passwordsave.content.t = 1  and not(Passwordsave.content.t=Tobecleaned) 
	\#Repassword.content.t = 1  and not(Repassword.content.t=Tobecleaned)
	all iw: Field| (iw in Propertyrequired.requireds) => \#iw.content.t = 1 and not(iw.content.t=Tobecleaned)
}
pred uniquefieldstest [t: Time] {
	all o: List.elements.t | (\#o.vs.Usersave= 1 => Usersave.content.t !=o.vs.Usersave)
}
\end{lstlisting}
}


==> listings/CRUD.tex <==
{
\begin{lstlisting}[language=Alloy,caption={CRUD Abstract Semantics model}]
--------------------Initial State---------------
pred init [t: Time] {
	no Selectablewidget.list.t
	no Track.op.t
	no Selectablewidget.selected.t
 	Currentwindow.isin.t = sws.Selectablewidget
	\#Createtrigger = 0 =>Currentcrudop.operation.t = CREATE else \#Currentcrudop.operation.t = 0
	\#Tobecleaned = 1
	all iw: Inputwidget | \#iw.content.(T/first) > 0
}
---------------Generic CRUD Structure ----------
abstract sig Ok, Cancel extends Actionwidget { }
abstract sig Createtrigger extends Actionwidget { }
abstract sig Updatetrigger extends Actionwidget { }
abstract sig Deletetrigger extends Actionwidget { }
fact {
	\#Ok < 2
	\#Selectablewidget = 1
	all iw: Inputwidget | not(iw.content.(T/first) = Tobecleaned) => not(iw in Propertysemantic.requireds) 
}
---------------Generic CRUD Semantics---------- 
abstract sig Crudop {}
one sig CREATE, UPDATE extends Crudop {}
one sig Currentcrudop {
	operation: Crudop lone -> Time
}
one sig Propertysemantic{
	uniques: set Inputwidget,
	requireds: set Inputwidget
} 
sig Objectinlist extends Object{
	vs: Value lone ->Inputwidget
}
pred fillsemantics [iw: Inputwidget, t: Time, v: Value] { }
pred fillsuccesspost [iw: Inputwidget, t, t': Time, v: Value] { 
	Currentcrudop.operation.t' = Currentcrudop.operation.t
}
pred fillfailpost [iw: Inputwidget, t, t': Time, v: Value] { 
	Currentcrudop.operation.t' = Currentcrudop.operation.t
}
pred fillpre[iw: Inputwidget, t: Time, v: Value] { 
	(\#iw.content.(T/first) = 1 and not(iw.content.(T/first) = Tobecleaned)) => not(v = none)
}
pred selectsemantics [sw: Selectablewidget, t: Time, o: Object] { }
pred selectfailpost [sw: Selectablewidget, t, t': Time, o: Object] {
	Currentcrudop.operation.t' = Currentcrudop.operation.t
	all iw: Inputwidget | iw.content.t' = iw.content.t
}
pred selectsuccesspost [sw: Selectablewidget, t, t': Time, o: Object] {
	\#Createtrigger = 0 => (Currentcrudop.operation.t' = UPDATE and loadform[o, t'])  else (\#Currentcrudop.operation.t' = 0 and all iw: Inputwidget | iw.content.t' = iw.content.t)
}
pred selectpre[sw: Selectablewidget, t: Time, o: Object] { 
	o in sw.list.t
}
pred clicksemantics [aw: Actionwidget, t: Time] {
	(aw in Ok and Currentcrudop.operation.t in CREATE) => filledrequiredtest [t] and uniquetest [t] 
	(aw in Ok and Currentcrudop.operation.t in UPDATE) => filledrequiredtest [t] and uniqueforupdatetest [t]
	(aw in Deletetrigger) => 2=(1+1)
}
pred clicksuccesspost [aw: Actionwidget, t, t': Time] {
	Currentwindow.isin.t' = aw.goes
	(aw in Createtrigger) => (Currentcrudop.operation.t' = CREATE and Selectablewidget.list.t' = Selectablewidget.list.t and (all iw: Inputwidget | iw.content.t' = iw.content.(T/first)) and \#Selectablewidget.selected.t' = 0)
	(aw in Updatetrigger) => (Currentcrudop.operation.t' = UPDATE and Selectablewidget.list.t' = Selectablewidget.list.t and loadform[Selectablewidget.selected.t, t']  and Selectablewidget.selected.t' = Selectablewidget.selected.t)
	(aw in Deletetrigger) => (\#Selectablewidget.selected.t' = 0 and delete [t, t'])
	(aw in Deletetrigger and \#Createtrigger = 0) => (Currentcrudop.operation.t' = CREATE  and (all iw: Inputwidget | iw.content.t' = iw.content.(T/first)))
	(aw in Deletetrigger and \#Createtrigger > 0) => (\#Currentcrudop.operation.t' = 0  and (all iw: Inputwidget | iw.content.t' = iw.content.(T/first)))	
	(aw in Cancel and \#Createtrigger > 0) => (\#Currentcrudop.operation.t' = 0 and Selectablewidget.list.t' = Selectablewidget.list.t and \#Selectablewidget.selected.t' = 0)
	(aw in Cancel and \#Createtrigger = 0) => (Currentcrudop.operation.t' = CREATE and Selectablewidget.list.t' = Selectablewidget.list.t and \#Selectablewidget.selected.t' = 0  and (all iw: Inputwidget | iw.content.t' = iw.content.(T/first)))
	
	(aw in Ok and Currentcrudop.operation.t in CREATE) => (\#Selectablewidget.selected.t' = 0 and add [t, t'])
	(aw in Ok and Currentcrudop.operation.t in UPDATE) => (\#Selectablewidget.selected.t' = 0 and update [t, t'])
	(aw in Ok and \#Createtrigger > 0) => (\#Currentcrudop.operation.t' =0)
	(aw in Ok and \#Createtrigger = 0) => (Currentcrudop.operation.t' =CREATE  and (all iw: Inputwidget | iw.content.t' = iw.content.(T/first)) and \#Selectablewidget.selected.t' = 0)
}
pred clickfailpost [aw: Actionwidget, t, t': Time]	{
	Selectablewidget.list.t' = Selectablewidget.list.t
	(all iw:Inputwidget | iw.content.t' = iw.content.t)
	Selectablewidget.selected.t' = Selectablewidget.selected.t
	Currentcrudop.operation.t' = Currentcrudop.operation.t
}
pred clickpre[aw: Actionwidget, t: Time] {
	(aw in Updatetrigger) => \#Selectablewidget.selected.t = 1
	(aw in Deletetrigger) => \#Selectablewidget.selected.t = 1
}
pred add [t, t': Time] {
	one o: Objectinlist |all iw: Inputwidget | not(o in Selectablewidget.list.t) and o.appeared = t' and (iw.content.t = Tobecleaned => \#o.vs.iw = 0 else o.vs.iw = iw.content.t) and Selectablewidget.list.t' = Selectablewidget.list.t+o
}
pred filledrequiredtest [t: Time] { 
	all iw: Propertysemantic.requireds|  not(iw.content.t = Tobecleaned) and not( \\#iw.content.t = 0)
}
pred  uniquetest [t: Time] { 
	all iw: Propertysemantic.uniques | all o: Selectablewidget.list.t | (\#(o.vs.iw)=1) => iw.content.t !=o.vs.iw
}
pred  uniqueforupdatetest [t: Time] {
	all iw: Propertysemantic.uniques | all o: (Selectablewidget.list.t-Selectablewidget.selected.t) |  (\#(o.vs.iw)=1) => iw.content.t !=o.vs.iw
}
pred loadform [o: Object, t': Time] {
	all iw: Inputwidget | iw.content.t' = o.vs.iw
}
pred update [t, t': Time] {
	one o: Object | all iw: Inputwidget | not(o in Selectablewidget.list.t) and o.appeared = Selectablewidget.selected.t.appeared and (iw.content.t = Tobecleaned => \#o.vs.iw = 0 else o.vs.iw = iw.content.t) and Selectablewidget.list.t' = (Selectablewidget.list.t - Selectablewidget.selected.t)+o
}
pred delete [t, t': Time] {
	Selectablewidget.list.t' = Selectablewidget.list.t - Selectablewidget.selected.t
}
\end{lstlisting}
}


==> listings/SAVE.tex <==
{
\begin{lstlisting}[language=Alloy,caption={SAVE Abstract Semantics model}]
--------------------Initial State---------------
pred init [t: Time] {
	no Track.op.t
	Currentwindow.isin.t = aws.New
	\#Openinglist.list.t = 0
	\#(Auxiliary.saved.t) = 1
	no Selectablewidget.selected.t
	\#Tobecleaned = 1
	all iw: Inputwidget | \#iw.content.(T/first) > 0
}
---------------Generic SAVE Structure ----------
abstract sig New, Open, Save, Saveas, Saves, Cancelsave, Openo, Cancelopen, Encryptb, Backe, Decryptb, Backd, Yes, No, Replace, Noreplace extends Actionwidget { }
abstract sig Filename, Password, Repassword, Depassword extends Inputwidget { }
abstract sig Openinglist extends Selectablewidget { }

---------------Generic SAVE Semantics---------- 
one sig Auxiliary{
	pwd: Object lone -> Value,
	haspwd: one Object,
	names: Object one -> Value,
	saved: Value lone -> Time
}
pred fillsemantics [iw: Inputwidget, t: Time, v: Value] {
	
}
pred fillsuccesspost [iw: Inputwidget, t, t': Time, v: Value] {
	Openinglist.list.t' =  Openinglist.list.t
	(Auxiliary.saved.t') = 	(Auxiliary.saved.t)
}
pred fillfailpost [iw: Inputwidget, t, t': Time, v: Value] {
	Openinglist.list.t' =  Openinglist.list.t
	(Auxiliary.saved.t') = 	(Auxiliary.saved.t)
}
pred fillpre [iw: Inputwidget, t: Time, v: Value] { }
pred selectsemantics [sw: Selectablewidget, t: Time, o: Object] {
	
}
pred selectsuccesspost [sw: Selectablewidget, t, t': Time, o: Object] {
	Openinglist.list.t' =  Openinglist.list.t
	(Auxiliary.saved.t') = 	(Auxiliary.saved.t)
	(all iw: Inputwidget | iw.content.t' = iw.content.t)
}
pred selectfailpost [sw: Selectablewidget, t, t': Time, o: Object] {
	Openinglist.list.t' =  Openinglist.list.t
	(Auxiliary.saved.t') = 	(Auxiliary.saved.t)
	(all iw: Inputwidget | iw.content.t' = iw.content.t)
}
pred selectpre [sw: Selectablewidget, t: Time, o: Object] { }
pred clicksemantics [aw: Actionwidget, t: Time] {
	(aw in Save)        => \#(Auxiliary.saved.t) = 0
	(aw in Openo)     => \#Openinglist.selected.t = 1
	(aw in Saves)      => \#Filename.content.t = 1 and not(Filename.content.t = Tobecleaned)
	(aw in Encryptb)   => Password.content.t = Repassword.content.t
	(aw in Decryptb) => Depassword.content.t = (Openinglist.selected.t).(Auxiliary.pwd)
}
pred clicksuccesspost [aw: Actionwidget, t, t': Time] {
	(aw in New and \#aw.goes = 0) => new[t,t']
	(aw in New and \#aw.goes > 0) => same[t,t'] and Currentwindow.isin.t' = aw.goes
	(aw in Open) => same[t,t'] and Currentwindow.isin.t' = aw.goes
	(aw in Save) => same[t,t'] and Currentwindow.isin.t' = aw.goes
	(aw in Saveas) => same[t,t'] and Currentwindow.isin.t' = aw.goes
	(aw in Saves and exisit[t, Filename.content.t]) => ((\#Replace = 1) => (Currentwindow.isin.t' = aws.Replace and same[t,t']) else ((\#Encryptb = 1 or \#Yes = 1) => (same[t,t'] and (\#Yes = 1 => Currentwindow.isin.t' = aws.Yes else Currentwindow.isin.t' = aws.Encryptb)) else (savenp[t,t', Filename.content.t])))
	(aw in Saves and not(exisit[t, Filename.content.t])) => ((\#Encryptb = 1 or \#Yes = 1) => (same[t,t'] and (\#Yes = 1 => Currentwindow.isin.t' = aws.Yes else Currentwindow.isin.t' = aws.Encryptb)) else (savenp[t,t', Filename.content.t]))
	(aw in Cancelsave) => returned[t, t']
	(aw in Openo) => ((Openinglist.selected.t) in (Auxiliary.haspwd)) => (Currentwindow.isin.t' = aws.Decryptb and same[t,t']) else (openo[t,t'])
	(aw in Cancelopen) => returned[t, t']
	(aw in Encryptb) => save[t,t', Password.content.t, Filename.content.t]
	(aw in Backe) => (\#Yes = 1) => savenp[t,t', Filename.content.t] else((aw.goes in aws.New) => returned[t,t'] else (same2[t,t'] and Currentwindow.isin.t' = aw.goes))
	(aw in Decryptb) => openo[t, t']
	(aw in Backd) => ((aw.goes in aws.New) => returned[t,t'] else (same2[t,t'] and Currentwindow.isin.t' = aw.goes))
	(aw in Yes) => same[t,t'] and Currentwindow.isin.t' = aw.goes
	(aw in No) => savenp[t,t', Filename.content.t]
	(aw in Replace) => ((\#Encryptb = 1 or \#Yes = 1) => (same[t,t'] and (\#Yes = 1 => Currentwindow.isin.t' = aws.Yes else Currentwindow.isin.t' = aws.Encryptb)) else (savenp[t,t', Filename.content.t]))
	(aw in Noreplace) => ((aw.goes in aws.New) => returned[t,t'] else (same2[t,t'] and Currentwindow.isin.t' = aw.goes))
}
pred clickfailpost [aw: Actionwidget, t, t': Time] {
	(aw in (Encryptb+Decryptb)) => (all iw: Inputwidget | iw.content.t' = iw.content.(T/first)) else (all iw: Inputwidget | iw.content.t' = iw.content.t)
	Openinglist.list.t' =  Openinglist.list.t
	Openinglist.selected.t' =  Openinglist.selected.t
	(Auxiliary.saved.t') = 	(Auxiliary.saved.t)
}
pred clickpre [aw: Actionwidget, t': Time] { }
pred save [t, t': Time, password, filename: Value] {
	(filename in (Openinglist.list.t).(Auxiliary.names)) => (one o: Object | o in Auxiliary.haspwd and not(o in Openinglist.list.t) and o.appeared = Auxiliary.names.filename.appeared and (password = Tobecleaned =>\#o.(Auxiliary.pwd)=0 else o.(Auxiliary.pwd) = password) and o.(Auxiliary.names) = filename and Openinglist.list.t' = (Openinglist.list.t - (Auxiliary.names).filename)+o) else (one o: Object | o in Auxiliary.haspwd and not(o in Openinglist.list.t) and o.(Auxiliary.pwd) = password and o.(Auxiliary.names) = filename and o.appeared = t' and Openinglist.list.t' = Openinglist.list.t + o)
	\#(Auxiliary.saved.t') = 1
	Currentwindow.isin.t' = aws.New
	\#Openinglist.selected.t' = 0
  (all iw: Inputwidget | iw.content.t' = iw.content.(T/first))
}
pred savenp [t, t': Time, filename: Value] {
	(filename in (Openinglist.list.t).(Auxiliary.names)) => (one o: Object | not(o in Auxiliary.haspwd) and not(o in Openinglist.list.t) and o.appeared = Auxiliary.names.filename.appeared and o.(Auxiliary.pwd) = none and o.(Auxiliary.names) = filename and Openinglist.list.t' = (Openinglist.list.t - (Auxiliary.names).filename)+o) else (one o: Object | not(o in Auxiliary.haspwd) and not(o in Openinglist.list.t) and o.(Auxiliary.pwd) = none and o.(Auxiliary.names) = filename and o.appeared = t' and	Openinglist.list.t' = Openinglist.list.t + o)
	\#(Auxiliary.saved.t') = 1
	Currentwindow.isin.t' = aws.New
	\#Openinglist.selected.t' = 0
	(all iw: Inputwidget | iw.content.t' = iw.content.(T/first))
}
pred new [t, t': Time] {
	\#(Auxiliary.saved.t') = 0
	(all iw: Inputwidget | iw.content.t' = iw.content.(T/first))
	Openinglist.list.t' =Openinglist.list.t
	\#Openinglist.selected.t' = 0
	Currentwindow.isin.t' = aws.New
}
pred openo [t, t': Time] {
	\#(Auxiliary.saved.t') = 1
	(all iw: Inputwidget | iw.content.t' = iw.content.(T/first))
	Openinglist.list.t' =  Openinglist.list.t
	Currentwindow.isin.t' = aws.New
	\#Openinglist.selected.t' = 0
}
pred exisit [t: Time, name: Value] {
	name in (Openinglist.list.t).(Auxiliary.names)
}
pred returned [t, t': Time] {
	(Auxiliary.saved.t') = 	(Auxiliary.saved.t)
	(all iw: Inputwidget | iw.content.t' = iw.content.(T/first))
	\#Openinglist.selected.t' = 0
	Openinglist.list.t' = Openinglist.list.t
	Currentwindow.isin.t' = aws.New
}

pred same [t, t': Time] {
	(Auxiliary.saved.t') = 	(Auxiliary.saved.t)
	(all iw:  Inputwidget | iw.content.t' = iw.content.t)
	Openinglist.selected.t' = Openinglist.selected.t
	Openinglist.list.t' = Openinglist.list.t
}
pred same2 [t, t': Time] {
	(Auxiliary.saved.t') = 	(Auxiliary.saved.t)
	(all iw: Inputwidget | iw.content.t' = iw.content.(T/first))
	Openinglist.selected.t' = Openinglist.selected.t
	Openinglist.list.t' = Openinglist.list.t
}
\end{lstlisting}
}


==> listings/alloymodel.tex <==
{
\begin{lstlisting}[language=Alloy,caption={Examples of Abstract Semantics model},captionpos=b]
/* GUI elements definition */
sig loginform, signupform, loggedpage extends Window{}
sig login, signup, register, logout extends Action_widget{}
sig user, pass, pass2,..., otherfields extends Input_widget{}
one sig Curr_win { /* Current window */
  is_in: Window one -> Time,
}
/* Functionality internal state elements */
sig Usr {
  username: one Value,
  password: one Value
}
sig Users{
  list: Usr set -> Time 
}
/* Semantic Property */
one sig Required{ 
  fields: set otherfields
}
pred preconditions [w: Widget, t: Time] {
  w in register=> not user.content.t=none && not pass.content.t=none &&
    (all us:Users.list.t | user.content.t!=us.username) &&
    pass.content.t=pass2 && (all iw:Required.fields | not iw.content.t=none)
}
pred postconditions [w: Widget, t,t': Time] {
  w in register=> one us:Users | us.username=user.content.t && 
    us.password=pass.content.t && Users.list.t'=Users.list.t+us &&
    (Curr_win.is_in.t'=loginform || Curr_win.is_in.t'=loggedpage)
}
\end{lstlisting}
\label{semantics}
}


==> listings/bug.tex <==
{
\begin{lstlisting}[caption={Faulty User Registration in OnShop},label={lst:bug},language=Java, firstnumber=300]
private void signup() {
  if (isValidForm()) {
     insertIntoDB();
     JOptionPane.showMessageDialog(SignupPanel, "Please Login to get Started!", "Congratulations", JOptionPane.DEFAULT_OPTION);<\Suppressnumber>
            ...<\Reactivatenumber{308}>
     card.show(this.getParent(), "startCard");//Return to Initial Window
  }else
     resetForm();
}<\Suppressnumber><\Reactivatenumber{315}>
private void insertIntoDB() {<\Suppressnumber>
            ... <\Reactivatenumber{334}>
  if (resultSet.next()) { //User Already Exists
     JOptionPane.showMessageDialog(SignupPanel,"Username already exists");
     resetForm();
  }
\end{lstlisting}
}

==> listings/general.tex <==
{
\begin{lstlisting}[language=Alloy,caption={Abstract Semantics model preamble},captionpos=b]
open util/ordering [Time] as T
open util/ternary
open util/relation
-----------------------Utils------------------------
sig Time { }
abstract sig Operation { }
sig Click extends Operation {
	clicked: one Actionwidget
}
sig Fill extends Operation {
	filled: one Inputwidget,
	with: lone Value
}
sig Select extends Operation {
	wid: one Selectablewidget,
	which: one Object
}
one sig Track { 
	op: Operation lone -> Time
}
pred transition [t, t': Time]  {
	(one aw: Actionwidget, c: Click | click [aw, t, t', c]) or 
	(one iw: Inputwidget, v: Value, f: Fill| fill [iw, t, t', v, f]) or
	(one iw: Inputwidget, f: Fill| fill [iw, t, t', none, f]) or	
	(one sw: Selectablewidget, s: Select, o: Object | select [sw, t, t', o, s]) 
}
pred System {
	init [T/first]
	all t: Time - T/last | transition [t, T/next[t]]
}
----------------Generic GUI Structure ----------------
abstract sig Window {
	aws: set Actionwidget,
	iws: set Inputwidget,
	sws: set Selectablewidget
}
abstract sig Actionwidget {
	goes: set Window
}
sig Value { }
one sig Optionvalue0 extends Value{ }
one sig Optionvalue1 extends Value{ }
one sig Optionvalue2 extends Value{ }
one sig Optionvalue3 extends Value{ }
one sig Optionvalue4 extends Value{ }
sig Tobecleaned extends Value{ }
abstract sig Inputwidget {
	content: Value lone -> Time,
	val: set Value
}
sig Object {
	appeared: one Time
}
abstract sig Selectablewidget {
	list: Object set -> Time,
	selected: Object lone ->Time
}
fact {
	\#Tobecleaned = 1 => not(Tobecleaned in Fill.with)
	all iw: Inputwidget | iw in Window.iws
	all aw: Actionwidget | aw in Window.aws
	all sw: Selectablewidget | sw in Window.sws
}
fact noredundant{
	no t: Time |  \#Track.op.t = 1 and Track.op.t in Fill and Track.op.t.with = Track.op.t.filled.content.(T/prev[t])
	no t: Time | \#Track.op.t = 1 and Track.op.t in Click and Track.op.(T/prev[t]) in Click and Track.op.t.clicked = Track.op.(T/prev[t]).clicked	
	no t: Time | \#Track.op.t = 1 and Track.op.t in Select and Track.op.(T/prev[t]) in Select and Track.op.(T/prev[t]).wid = Track.op.t.wid
	no t: Time | \#Track.op.t = 1 and Track.op.t in Fill and Track.op.(T/prev[t]) in Fill and Track.op.t.filled = Track.op.(T/prev[t]).filled
}
----------------Generic GUI Semantics ---------------
one sig Currentwindow {
	isin: Window one -> Time
}
pred click [aw: Actionwidget, t, t': Time, c: Click] {
	--- precondition ---
	aw in Currentwindow.isin.t.aws
	clickpre [aw, t]
	--- effect ---
	(clicksemantics [aw, t] and clicksuccesspost [aw, t, t']) or
	(not clicksemantics  [aw, t] and Currentwindow.isin.t' = Currentwindow.isin.t and clickfailpost [aw, t, t'])
	--- operation is tracked ---
	c.clicked = aw and Track.op.t' = c
}
pred fill [iw: Inputwidget, t, t': Time, v: Value, f: Fill] { 
	--- precondition ---
	(v = none)  => not(iw.content.t = Tobecleaned)
	iw in Currentwindow.isin.t.iws
	fillpre [iw, t, v]
	--- effect ---
	(fillsemantics  [iw, t, v] and iw.content.t' = v and fillsuccesspost [iw, t, t', v]) or
	(not fillsemantics  [iw, t, v] and iw.content.t' = iw.content.t and fillfailpost [iw, t, t', v])
	--- general postcondition ---
	Currentwindow.isin.t' = Currentwindow.isin.t
	all iww: (Inputwidget - iw) | iww.content.t' = iww.content.t
	all sw:Selectablewidget | sw.selected.t' = sw.selected.t and sw.list.t' = sw.list.t
	--- operation is tracked ---
	f.filled = iw and f.with = v and Track.op.t' = f
}
pred select [sw: Selectablewidget, t, t': Time, o: Object, s: Select] { 
	--- precondition ---
	sw in Currentwindow.isin.t.sws
	o in sw.list.t
	selectpre [sw, t, o]
	--- effect ---
	(selectsemantics  [sw, t, o] and sw.selected.t' = o and selectsuccesspost [sw, t, t', o]) or
	(not selectsemantics  [sw, t, o] and sw.selected.t' = sw.selected.t and selectfailpost [sw, t, t', o])
	--- general postcondition ---
	Currentwindow.isin.t' = Currentwindow.isin.t
	all sww: (Selectablewidget - sw) | sww.selected.t' = sww.selected.t and sww.list.t' = sww.list.t
	sw.list.t' = sw.list.t	
	--- operation is tracked ---
	s.wid = sw and s.which = o and Track.op.t' = s
}
\end{lstlisting}
}


==> listings/ordering.tex <==
{
\begin{lstlisting}[language=Java,caption={Weak event ordering computation algorithm},captionpos=b]
past = map<Event, List<Event>
prevE = null
for(i = 0 : n+1){
	s = GUIstates[i+1]
	e = events[i]
	if(enabled(prevE, s)){
		past(e) = past(prevE)
	}else{
		past(e) = events[0, i]
	}	
	prevE = e
}
\end{lstlisting}
\label{ordering}
}


==> listings/search.tex <==
\begin{lstlisting}[language=java, caption={GUI Pattern Matching Algorithm}, label={match.alg}]
List<GUIPatternMatch> match(GUI g, GUIPattern p)
	for(Window w: g.getWindows())
		GUIPatternMatch match = traverse(w, firstPatternWindow, new GUIPatternMatch())
		if(match != null && isValidMatch(match))
			outlist.add(match)
	return outlist

GUIPatternMatch traverse(Window w,  Pattern_window pw, GUIPatternMatch m)
	if (m.containsMatch(pw, w)
		return m;
	WindowMatch win_match = match_window(w, pw)
	if (win_match == null)
		return null
	m.add(win_match)
		
	for (Pattern_action_widget paw : pw.getActionWidgets()) 
		Action_widget aw = win_match.getMatchedAW(paw)
		for (Pattern_window target : getForwardPatternEdges(paw))			
			for (Window reached : getForwardEdges(aw))
				GUIPatternMatch new_match = traverse(reached, target, m)
				if(new_match == null && isRequired(target))
					return null
				m = new_match
	return m
\end{lstlisting}

==> listings/structuralrefinement.tex <==
\begin{lstlisting}[language=java, caption={Refinement Algorithm}, label={struct.alg}]
GUIPatternMatch refine(GUIPatternMatch match, GUIPattern p)
	do //edge and windows refinement
		for(Edge e:p.getDynamicEdges())
			GUITestcase tc = generateTestcaseToCoverEdge(match, e)
			runGUITestcase(tc)
			if(edgeIsCovered())
				match.addEdge(e)
			else
				match.updateSemanticProperties()
	
		for(Pattern_window pw: undiscoveredWindows(match, p))
			GUITestcase tc = generateTestcaseToOpenWindow(match, pw)
			runGUITestcase(tc)
			if(windowIsFound())
				match.addWindow(w)
			else
				match.updateSemanticProperties()	
	while(!nothingMoreToDiscover && !nothingWasDiscoveredInThisIteration)
	
	do //semantic property refinement
		GUITestcase tc = generateTestcase(match)
		runGUITestcase(tc)
		if(!behaviorWasConsistent)
			match.updateSemanticProperties()	
	while(!timeout || semanticPropertyConverged)
	
	return match
\end{lstlisting}
